Enhancing Adversarial Transferability in Visual-Language Pre-training Models via Local Shuffle and Sample-based Attack

Visual-Language Pre-training (VLP) models have achieved significant performance across various downstream tasks. However, they remain vulnerable to adversarial examples. While prior efforts focus on improving the adversarial transferability of multimodal adversarial examples through cross-modal interactions, these approaches suffer from overfitting issues, due to a lack of input diversity by relying excessively on information from adversarial examples in one modality when crafting attacks in another. To address this issue, we draw inspiration from strategies in some adversarial training methods and propose a novel attack called Local Shuffle and Sample-based Attack (LSSA). LSSA randomly shuffles one of the local image blocks, thus expanding the original image-text pairs, generating adversarial images, and sampling around them. Then, it utilizes both the original and sampled images to generate the adversarial texts. Extensive experiments on multiple models and datasets demonstrate that LSSA significantly enhances the transferability of multimodal adversarial examples across diverse VLP models and downstream tasks. Moreover, LSSA outperforms other advanced attacks on Large Vision-Language Models.

==> EMNLP2024/resubmit.tex <==
Changed of Resubmission
In the previous review cycle, the AC noted that "However, as the reviewers pointed out, a more detailed analysis of why the LSSA enhances transferability is required; additional discussions or comparisons with the existing literature would be beneficial to substantiate its novelty and effectiveness." In response to this, we have expanded our description of the reasons in Section 1 (line 60-84) and Section 3 (line 312-330), introducing the distinctions between LSSA and existing methods, allowing reviewers to better understand the innovation and efficacy of LSSA.

The three reviewers primarily raised the following issues:
1. The novelty of conception.
2. The example depicted in Figure 2 is not sufficiently representative, making it challenging to comprehend the specific intricacies of the method.
3. There are too few contributions. Contributions 1 and 2 are essentially the same, with Contribution 1 merely outlining existing problems.
4. Due to the absence of specific visualizations, it is unclear what the adversarial samples generated by LSSA appear like.
5. The notations used from Line 292 to 300, and in Algorithm 1 are inconsistent, which can cause confuse. For example, v in line 296 is supposed to be dependent on i. In algorithm 1, it is unclear where j and M are used.

For question 1, we reintroduce our contributions in Section 1 (line 110-115) and highlight the differences in Section 3 (line 312-330). It allows reviewers to know more clearly the difference between LSSA and existing methods.

For question 2, we modify the content of the schematic diagram (Figure 2). We add the shuffled images to represent the operations performed, and the step number is added according to the order.

For question 3, we rewrite the first contribution (line 110-115) to claim our observations, which is different from the second contribution. We revisit our observations, refine the underlying reasons, and present our first contribution more clearly.

For question 4, we add a reference (line 242) to the appendix (line 715-722) in the content to make the reviewer understand the difference between original and adversarial image-text pairs by visualizations.

For question 5, we correct the formatting errors present in the previous version of the paper. Specifically, we have kept the variable names used in Section 3 (line 292-300) consistent with those in the appendix (line 732-734) so that reviewers can better understand the algorithm process.

Moreover, we have also made other changes to make the reviewers' reading experience better and reduce typos.
